Validation of Semi-Empirical xTB Methods for High-Throughput Screening of TADF Emitters: A 747-Molecule Benchmark Study

Thermally activated delayed fluorescence (TADF) emitters are essential for next-generation, high-efficiency organic light-emitting diodes (OLEDs), yet their rational design is hampered by the high computational cost of accurate excited-state predictions. Here, we present a comprehensive benchmark study validating semi-empirical extended tight-binding (xTB) methods -- specifically sTDA-xTB and sTD-DFT-xTB -- for the high-throughput screening of TADF materials. Using an unprecedentedly large dataset of \num{747} experimentally characterized emitters, our framework demonstrates a computational cost reduction of over \qty{99}{\percent} compared to conventional TD-DFT, while maintaining strong internal consistency between methods (Pearson $r \approx \num{0.82}$ for \deltaest), validating their utility for relative molecular ranking. Validation against \num{312} experimental \deltaest values reveals a mean absolute error of approximately \qty{0.17}{\electronvolt}, a discrepancy attributed to the vertical approximation inherent to the HTS protocol, underscoring the methods' role in screening rather than quantitative prediction. Through large-scale data analysis, we statistically validate key design principles, confirming the superior performance of Donor-Acceptor-Donor (D-A-D) architectures and identifying an optimal D-A torsional angle range of \qtyrange{50}{90}{\degree} for efficient TADF. Principal Component Analysis reveals that the complex property space is fundamentally low-dimensional, with three components capturing nearly \qty{90}{\percent} of the variance. This work establishes these semi-empirical methods as powerful, cost-effective tools for accelerating TADF discovery and provides a robust set of data-driven design rules and methodological guidelines for the computational materials science community.

==> tables/table_comparative_summary.tex <==
\begin{table}[htbp]
\centering
\caption{Comparative performance summary of computational methods. The table shows the best performing method for each property and metric.}
\label{tab:comparative-summary}
\begin{tabular}{lcccc}
	\hline
	\textbf{Property} & \textbf{Best MAE} & \textbf{Best RMSE} & \textbf{Best R$^2$} & \textbf{Best Pearson r} \\ \hline
	$\lambda_{PL}$    &   sTD-DFT (Tol)   &   sTD-DFT (Tol)    &    sTD-DFT (Tol)    &      sTD-DFT (Tol)      \\
	(nm)              &       78.76       &       118.76       &       -1.2498       &         0.6922          \\ \hline
	$\Delta E_{ST}$   &   sTD-DFT (Gas)   &   sTD-DFT (Gas)    &    sTD-DFT (Gas)    &      sTD-DFT (Gas)      \\
	(eV)              &      0.1680       &       0.3635       &       -0.0493       &         0.1827          \\ \hline
\end{tabular}
\end{table}

==> tables/table_emission_wavelength_metrics.tex <==
\begin{table}[htbp]
\centering
\caption{Statistical metrics for emission wavelength predictions (\(\lambda_{\mathrm{PL}}\)) comparing sTDA and sTD-DFT methods in gas and toluene phases against experimental/computational literature values (N=213 molecules).}
\label{tab:emission-wavelength-metrics}
\begin{tabular}{lccccc}
	\hline
	\textbf{Method}   & \textbf{MAE (nm)} & \textbf{RMSE (nm)} & \(\mathbf{R^2}\) & \textbf{Pearson \(r\)} & \textbf{\(p\)-value} \\ \hline
	sTDA (Gas)        &       89.2        &       149.0        &      -2.54       &         0.561          &       4.50e-19       \\
	sTD-DFT (Gas)     &       85.3        &       135.4        &      -1.93       &         0.630          &       5.94e-25       \\
	sTDA (Toluene)    &       80.7        &       124.0        &      -1.45       &         0.663          &       2.48e-28       \\
	sTD-DFT (Toluene) &       78.8        &       118.8        &      -1.25       &         0.692          &       1.02e-31       \\ \hline
\end{tabular}
\end{table}

==> tables/table_pl_metrics.tex <==
\begin{table}[htbp]
\centering
\caption{Statistical metrics for Photoluminescence Wavelength predictions. Comparison of sTDA and sTD-DFT methods in gas phase and toluene phase against reference data from literature.}
\label{tab:table-pl-metrics}
\begin{tabular}{lccccccc}
	\hline
	\textbf{Method} & \textbf{N} & \textbf{MAE} & \textbf{RMSE} & \textbf{R$^2$} & \textbf{Pearson r} & \textbf{MAPE} & \textbf{Max Error} \\
	                &            &     (nm)     &     (nm)      &                &                    &     (\%)      &        (nm)        \\ \hline
	sTDA Gas        &    213     &    89.24     &    149.01     &    -2.5419     &       0.5612       &     17.7      &       684.89       \\
	sTD-DFT Gas     &    213     &    85.28     &    135.43     &    -1.9257     &       0.6299       &     16.6      &       621.59       \\
	sTDA Tol        &    213     &    80.68     &    124.03     &    -1.4538     &       0.6629       &     15.7      &       495.89       \\
	sTD-DFT Tol     &    213     &    78.76     &    118.76     &    -1.2498     &       0.6922       &     15.2      &       474.81       \\ \hline
\end{tabular}
\end{table}

==> tables/table_st_gap_metrics.tex <==
\begin{table}[htbp]
\centering
\caption{Statistical metrics for singlet-triplet energy gap predictions (\(\Delta E_{\mathrm{ST}}\)) comparing sTDA and sTD-DFT methods in gas and toluene phases against experimental/computational literature values (N=296 molecules).}
\label{tab:st-gap-metrics}
\begin{tabular}{lccccc}
	\hline
	\textbf{Method}   & \textbf{MAE (eV)} & \textbf{RMSE (eV)} & \(\mathbf{R^2}\) & \textbf{Pearson \(r\)} & \textbf{\(p\)-value} \\ \hline
	sTDA (Gas)        &       0.174       &       0.367        &      -0.07       &         0.181          &       1.80e-03       \\
	sTD-DFT (Gas)     &       0.168       &       0.364        &      -0.05       &         0.183          &       1.60e-03       \\
	sTDA (Toluene)    &       0.188       &       0.376        &      -0.12       &         0.161          &       5.39e-03       \\
	sTD-DFT (Toluene) &       0.183       &       0.377        &      -0.13       &         0.147          &       1.11e-02       \\ \hline
\end{tabular}
\end{table}

==> tables/table_st_metrics.tex <==
\begin{table}[htbp]
\centering
\caption{Statistical metrics for Singlet-Triplet Energy Gap predictions. Comparison of sTDA and sTD-DFT methods in gas phase and toluene phase against reference data from literature.}
\label{tab:table-st-metrics}
\begin{tabular}{lccccccc}
	\hline
	\textbf{Method} & \textbf{N} & \textbf{MAE} & \textbf{RMSE} & \textbf{R$^2$} & \textbf{Pearson r} & \textbf{MAPE} & \textbf{Max Error} \\
	                &            &     (eV)     &     (eV)      &                &                    &     (\%)      &        (eV)        \\ \hline
	sTDA Gas        &    296     &     0.17     &     0.37      &    -0.0695     &       0.1807       &      inf      &        5.21        \\
	sTD-DFT Gas     &    296     &     0.17     &     0.36      &    -0.0493     &       0.1827       &      inf      &        5.20        \\
	sTDA Tol        &    296     &     0.19     &     0.38      &    -0.1232     &       0.1614       &      inf      &        5.23        \\
	sTD-DFT Tol     &    296     &     0.18     &     0.38      &    -0.1285     &       0.1475       &      inf      &        5.22        \\ \hline
\end{tabular}
\end{table}

==> tables/table_validation_examples.tex <==
\begin{table}[htbp]
\centering
\caption{Representative examples from the emission wavelength validation dataset.
Molecules are selected to span the full range of prediction errors. Complete validation
dataset is provided in Supplementary \Cref{tab:supp-emission-complete,tab:supp-st-complete}.}
% S1 and S2
\label{tab:validation-examples}
\small
\begin{tabular}{lcccccc}
	\hline
	\textbf{Molecule} & \textbf{sTDA}  & \textbf{sTD-DFT} & \textbf{sTDA}  & \textbf{sTD-DFT} & \textbf{Ref.} &                 \textbf{Ref.}                 \\
	                  & \textbf{(Gas)} &  \textbf{(Gas)}  & \textbf{(Tol)} &  \textbf{(Tol)}  & \textbf{(nm)} &                                               \\ \hline
	DCzBNPh-1         &     472.4      &      475.7       &     442.1      &      445.7       &     472.5     &                \cite{Yan_2022}                \\
	BACH              &     433.6      &      439.5       &     409.9      &      415.7       &     427.7     &  \cite{Li_2022_10_1016_j_dyepig_2021_110030}  \\
	PyDCN–DMAC        &     508.7      &      504.4       &     496.9      &      493.2       &     494.2     &               \cite{Dong_2022}                \\
	tCTM              &     483.8      &      487.0       &     483.3      &      483.5       &     459.0     &                \cite{Tan_2020}                \\
	t-DABNA           &     431.1      &      438.5       &     418.4      &      425.5       &     464.0     &      \cite{Lee_2019_10_1039_c9tc02746g}       \\
	TPBPPI-PBI        &     472.9      &      473.4       &     461.4      &      462.6       &     429.0     &                \cite{Zhu_2020}                \\
	2Cz-DMAC-BTB      &     474.2      &      471.3       &     535.1      &      531.4       &     529.0     & \cite{Zhang_2022_10_1016_j_cclet_2021_08_064} \\
	TBPe              &     542.6      &      553.7       &     500.3      &      510.7       &     471.0     &                \cite{Yao_2019}                \\
	DPCN              &     511.7      &      511.6       &     508.0      &      508.3       &     424.0     & \cite{Xiao_2022_10_1016_j_dyepig_2022_110451} \\
	TRZ-3SO2          &     577.4      &      572.9       &     540.6      &      539.9       &     706.0     &     \cite{Zhang_2022_10_1039_d2tc02694e}      \\
	SBDBQ-PXZ         &     843.2      &      845.7       &     751.8      &      753.8       &     594.0     &                \cite{Yu_2018}                 \\
	{[2,1-b]IF}       &     1031.9     &      586.3       &     770.2      &      571.9       &     347.0     &              \cite{Romain_2016}               \\ \hline
	\multicolumn{7}{l}{\footnotesize Complete dataset: 213 molecules (emission), 296 molecules (ST gap)}
\end{tabular}
\end{table}

